Low-Rank Matrix Estimation From Rank-One Projections by Unlifted Convex Optimization

We study an estimator with a convex formulation for recovery of low-rank matrices from rank-one projections. Using initial estimates of the factors of the target $d_1\times d_2$ matrix of rank-$r$, the estimator admits a practical subgradient method operating in a space of dimension $r(d_1+d_2)$. This property makes the estimator significantly more scalable than the convex estimators based on lifting and semidefinite programming. Furthermore, we present a streamlined analysis for exact recovery under the real Gaussian measurement model, as well as the partially derandomized measurement model by using the spherical $t$-design. We show that under both models the estimator succeeds, with high probability, if the number of measurements exceeds $r^2 (d_1+d_2)$ up to some logarithmic factors. This sample complexity improves on the existing results for nonconvex iterative algorithms.

==> macros.tex <==
\RequirePackage{mathrsfs}
\RequirePackage{xcolor}
\PassOptionsToPackage{dvipsnames}{xcolor}
\RequirePackage{tcolorbox}
\RequirePackage{bm}
\RequirePackage[bb=boondox]{mathalfa}

\global\long\def\mb#1{\hm{#1}}
\global\long\def\mbb#1{\mathbb{#1}}
\global\long\def\mc#1{\mathcal{#1}}
\global\long\def\mcc#1{\mathscr{#1}}
\global\long\def\mr#1{\mathrm{#1}}
\global\long\def\msf#1{\mathsf{#1}}
\global\long\def\mfk#1{\mathfrak{#1}}
\global\long\def\E{\mbb E}
\global\long\def\P{\mbb P}
\global\long\def\var{\ensuremath{\mr{var}}}
\global\long\def\T{{\scriptscriptstyle{\textup{\textsf{T}}}}} %{{\scalebox{0.55}{\ensuremath{\msf T}}}}
\global\long\def\F{{\scriptstyle{\textup{F}}}} %{{\scalebox{0.55}{\ensuremath{\mr F}}}}
\global\long\def\d{\ensuremath{\mr d}}
\global\long\def\tr{\ensuremath{\mr{tr}}}
\global\long\def\supp{\ensuremath{\,\mr{supp}}}
\global\long\def\sgn{\ensuremath{\,\mr{sgn}}}
\global\long\def\argmax{\operatorname*{argmax}}
\global\long\def\argmin{\operatorname*{argmin}}
\global\long\def\Arg{\operatorname*{Arg}}
\global\long\def\defeq{\stackrel{\textup{\tiny def}}{=}}
\global\long\def\bbone{\mbb 1}
\global\long\def\norm#1{{\left\lVert #1\right\rVert }}
\global\long\def\inp#1{{\langle#1\rangle}}%
\global\long\def\conj#1{\overline{#1}}

\let\stk\st
\let\st\relax
\newcommand*{\st}[1][\colon]{\ifstrequal{#1}{\colon}{#1}{\,#1\,}}%
\renewcommand{\hat}[1]{\widehat{#1}}
\renewcommand{\tilde}[1]{\widetilde{#1}}
\renewcommand{\bar}[1]{\overline{#1}}
\newcommand{\ubar}[1]{\underline{#1}}%

\newcommand*{\bmx}[1]{%
{
\begin{bmatrix}
	#1
\end{bmatrix}
%
}}

% \newcommand{\alert}[1]{\textcolor{Cerulean}{\textbf{#1}}}
\RequirePackage{tcolorbox}
\tcbuselibrary{skins, breakable}
\newcommand{\notebox}[2][Note]{
        \begin{tcolorbox}[  title={#1} , 
                            coltitle=black, 
                            colbacktitle=yellow!80!white, 
                            colback=yellow!30!white,
                            text width = 0.75\linewidth,
                            boxrule  = 0pt,
                            fonttitle=\small\bfseries, 
                            fontupper=\footnotesize]
        #2
    \end{tcolorbox}
}

\newcommand{\thmbox}[1]{
		\begin{tcolorbox}[	breakable, 
							enhanced, 
							frame hidden,
							capture=minipage,
							colback=Dandelion!40!yellow!20!white] %green!60!blue!10!white
		{}%
		#1
		\end{tcolorbox}

}
